Detecting relevant changes in the spatiotemporal mean function

For a spatiotemporal process $\{X_j(s,t) | ~s \in S~,~t \in T \}_{j =1, \ldots , n} $, where $S$ denotes the set of spatial locations and $T$ the time domain, we consider the problem of testing for a change in the sequence of mean functions. In contrast to most of the literature we are not interested in arbitrarily small changes, but only in changes with a norm exceeding a given threshold. Asymptotically distribution free tests are proposed, which do not require the estimation of the long-run spatiotemporal covariance structure. In particular we consider a fully functional approach and a test based on the cumulative sum paradigm, investigate the large sample properties of the corresponding test statistics and study their finite sample properties by means of simulation study.

==> intro_proj.tex <==
\red{parameter $d$}

\begin{ass}\label{ass_4th}
    $\cbr{X_j}_{j \in \mathbb{Z}}$ satisfies (A1) and (A2) in assumption \ref{ass_2nd}. Furthermore, $\cbr{X_j}_{j \in \mathbb{Z}}$ satisfies
    \begin{enumerate}
        \item[(A3')] For all $j \in \mathbb{Z}$ there exists some $\psi \in \br{0,1}$ such that $\e \norm{\eta_j}^{4 + \psi} < \infty$.
        
        \item[(A4')] The sequence $\cbr{\eta_j}_{j \in \mathbb{Z}}$ can be approximated by $m$-dependent sequences $\cbr{\eta_{j,m}}_{j \in \mathbb{Z}}$ in the sense that for some $\kappa > 4 + \psi$ $$\sum_{m=1}^\infty \br{\e \norm{\eta_0 - \eta_{0,m} }^{4 + \psi} }^{1/\kappa} < \infty,$$
        where $\eta_{j,m}$ is defined by
        \begin{align*}
            \eta_{j,m} (s,t) = f(\varepsilon_j (s,t), ..., \varepsilon_{j-m+1} (s,t), \mathbf{\varepsilon}^*_{j,m} (s,t))
        \end{align*}
        with $\mathbf{\varepsilon}^*_{j,m} (s,t) = (\varepsilon^*_{j,m,j-m} (s,t), \varepsilon^*_{j,m,j-m-1} (s,t), ...),$ where $\varepsilon^*_{j,m,k}$ are i.i.d copies of $\varepsilon_0$ and independent of $\br{\varepsilon_j}_{j \in \mathbb{Z}}$.
    \end{enumerate}
\end{ass}

\red{
\begin{align*}
    \overline{X}_n := \frac{1}{n} \sum_{i=1}^n X_i
\end{align*}
}

In this chapter, we need to work with the eigenelements $\lambda_1, \lambda_2, ...$ and $v_1, v_2, ...$ of the covariance operator $C$ of $\cbr{X_j}_{j \in \mathbb{Z}}$. The covariance operator is defined by
\begin{align*}
    C(x) (s_1, t_1) := \sum_{s_2 \in S} \int c \br{(s_1, t_1), (s_2, t_2)} x(s_2, t_2) \mathrm{d}t_2,
\end{align*}
where the covariance function $c$ is defined by
\begin{align*}
    c\br{(s_1, t_1), (s_2, t_2)} := \E{(X_0(s_1, t_1) - \mu (s_1, t_1)) (X_0(s_2, t_2) - \mu (s_2, t_2))}.
\end{align*}
For this, we need the following assumption:

\begin{ass}\label{eigvals_order}
    There exists a $d \in \mathbb{N}$, such that $\lambda_1 > \cdots > \lambda_d > \lambda_{d+1} > 0$.
\end{ass}

We estimate the eigenelements by the eigenelements of the empirical covariance operator of a subsample $X_1, ..., X_{\gbr{n\lambda}}$ for some $\lambda \in \sqbr{0,1}$, which is defined as
\begin{align*}
    \hat{C}_{n, \lambda} (x) (s_1, t_1) := \sum_{s_2 \in S} \int \hat{c}_{n, \lambda} \br{ (s_1, t_1) , (s_2, t_2)} x \br{(s_2, t_2)} \mathrm{d}t_2
\end{align*}
for $x \in L^2(S \times \sqbr{0,1})$ and $t_1 \in \sqbr{0,1}$, where
\begin{align*}
    \hat{c}_{n, \lambda} \br{(s_1, t_2), (s_2, t_2)} := \frac{1}{\gbr{n \lambda}} \sum_{i=1}^{\gbr{n \lambda}} (X_i(s_1, t_1) - \hat{\mu}_{n, \lambda} (s_1, t_1)) (X_i(s_2, t_2) - \hat{\mu}_{n, \lambda} (s_2, t_2)).
\end{align*}
and $$\hat{\mu}_{n, \lambda} := \frac{1}{\gbr{n \lambda}} \sum_{i=1}^{\gbr{n \lambda}} X_i.$$
We denote by $\hat{\lambda}_{1, \lambda}, \hat{\lambda}_{2,\lambda}, ...$ and $\hat{v}_{1, \lambda}, \hat{v}_{2, \lambda}, ...$ the eigenelements of $\hat{C}_{n,\lambda}$.

==> intro_spatiotemp.tex <==
Let $\cbr{X_j}_{j \in \mathbb{Z}}$ be a sequence of square integrable random functions on $S \times T$, where $T$ denotes a compact interval on $\mathbb{R}$. For sake of simplicity, we assume that $T=\sqbr{0,1}$. The set $S$ is a finite subset from $\mathbb{R}^z$ for some $z \in \mathbb{N}$.

We denote by $\norm{\cdot}$ the $L^2 (S \times T)$ norm induced by the inner product $\innpr{f,g} = \sum_{s \in S} \int_T f(s, t) g(s, t) \mathrm{d}t$.

In order to prove the results in the next section, we need to make the following assumptions:

\begin{ass}\label{ass_2nd}\,
    \begin{enumerate}
        \item[(A1)] For $j \in \mathbb{Z}$, we have $X_j = \mu + \eta_j$ with $\cbr{\eta_j}_{j \in \mathbb{Z}}$, where $\mu \in L^2 (S \times \sqbr{0,1})$ and $\cbr{\eta_j}_{j \in \mathbb{Z}}$ is a centered error process which satisfies (A2)-(A4).
        
        \item[(A2)] $\cbr{\eta_j}_{j \in \mathbb{Z}}$ forms a sequence of Bernoulli shifts, i.e. there exist a measurable space $\mathpcal{S}$, a measurable function $f : \mathpcal{S}^\infty \longrightarrow L^2 (S \times \sqbr{0,1})$ and a sequence of i.i.d $\mathpcal{S}$-valued functions $\cbr{\varepsilon_j}_{j \in \mathbb{Z}}$ such that $$\eta_j (s,t) = f(\varepsilon_j (s,t), \varepsilon_{j-1} (s,t), ...) \pppad \text{for all } j \in \mathbb{Z}$$
        and $\varepsilon_j (s,t) = \varepsilon_j (s, t, \omega)$ is jointly measurable in $(s, t, \omega)$ for $j \in \mathbb{Z}$.

        \item[(A3)] For all $j \in \mathbb{Z}$ there exists some $\psi \in \br{0,1}$ such that $\e \norm{\eta_j}^{2 + \psi} < \infty$.
        
        \item[(A4)] The sequence $\cbr{\eta_j}_{j \in \mathbb{Z}}$ can be approximated by $m$-dependent sequences $\cbr{\eta_{j,m}}_{j \in \mathbb{Z}}$ in the sense that for some $\kappa > 2 + \psi$ $$\sum_{m=1}^\infty \br{\e \norm{\eta_0 - \eta_{0,m} }^{2 + \psi} }^{1/\kappa} < \infty,$$
        where $\eta_{j,m}$ is defined by
        \begin{align*}
            \eta_{j,m} (s,t) = f(\varepsilon_j (s,t), ..., \varepsilon_{j-m+1} (s,t), \mathbf{\varepsilon}^*_{j,m} (s,t))
        \end{align*}
        with $\mathbf{\varepsilon}^*_{j,m} (s,t) = (\varepsilon^*_{j,m,j-m} (s,t), \varepsilon^*_{j,m,j-m-1} (s,t), ...),$ where $\varepsilon^*_{j,m,k}$ are i.i.d copies of $\varepsilon_0$ and independent of $\cbr{\varepsilon_j}_{j \in \mathbb{Z}}$.
    \end{enumerate}
\end{ass}

These assumptions are different from \cite{gromenko}, who assumed the random variables $\eta_j$ to be independent and identically distributed. Moreover, they make the assumption of seperability concerning the spatio-temporal variance structure, which means that it factors into a purely spatial and a purely temporal component.

==> proj_cp_mean.tex <==

For change point detection, we recall the model from the previous paragraph
\begin{align*}
    X_i = \begin{cases}
        \mu + f_1 (\varepsilon_i, \varepsilon_{i-1}, ...), & i \leq n \vartheta_0,\\
        \mu + \delta + f_2 (\varepsilon_i, \varepsilon_{i-1}, ...), & i > n \vartheta_0.\\
    \end{cases}
\end{align*}
In this chapter, we want to test the hypotheses
\begin{center}
    $H_0: \norm{\delta}^2 \leq \Delta$ vs. $H_1: \norm{\delta}^2 > \Delta$.
\end{center}

\noindent To this end, we use the same estimator for the change point as in the previous chapter, which was defined in (\ref{def_changepoint_estimator}).

% We first define the estimator for the unknown change point $\vartheta_0$
%\begin{align}\label{def_changepoint_estimator_2}
%    \hat{\vartheta} := \frac{1}{n} \argmax_{\gbr{n \varepsilon} + 1 \leq k \leq n - \gbr{n \varepsilon}} f (k),
%\end{align}
%where $\varepsilon \in [0, 1/2)$ and
%\begin{align*}
%    f(k) := \frac{k(n-k)}{n^2} \norm{\frac{1}{k} \sum_{i=1}^k X_i \otimes X_i - \frac{1}{n-k} \sum_{i= k+1}^n X_i \otimes X_i}^2_2
%\end{align*}

%\begin{prop}\label{prop:changepoint_conv_rate}
%    Under assumption \ref{ass_4th}, $\norm{\delta}^2 > 0$ and $\vartheta_0 \in (\varepsilon, 1- \varepsilon)$, then $$\hat{\vartheta} = \vartheta_0 + o_\p (n^{-1/2}).$$
%\end{prop}
%\begin{proof}
%    The proof follows the same two steps as in the proof of Proposition 3.1 in \cite{dette}. Since the first step is slightly different, we give the differing part. The convergence
%    $$\cbr{\sqrt{n} (f (\gbr{n \vartheta}) - d(\vartheta))}_{\vartheta \in \sqbr{0,1}} \convproc \cbr{\mathbb{G} (\vartheta)}_{\vartheta \in \sqbr{0,1}},$$ where $$d (\vartheta) := \vartheta (1-\vartheta) \norm{c^{(1)} + \mu \otimes \mu - (c^{(2)} + (\mu + \delta) \otimes (\mu + \delta)) }^2_2 \begin{cases}
%        \br{\frac{1-\vartheta_0}{1-\vartheta}}^2, & 0 < \vartheta \leq \vartheta_0\\
%        \br{\frac{\vartheta_0}{\vartheta}}^2, & \vartheta_0 < \vartheta < 1
%    \end{cases}$$
%    must be shown, where $c^{(i)}$ is the covariance function of $\eta_0^{(i)}$ for $i=1,2$. However, this follows by exactly the same arguments as in the proof of Proposition 3.1 in \cite{dette}.
%\end{proof}

In this scenario, it is possible that the covariance function will not be the same before and after the change point, leading to the fact that we have two covariance functions. This means that we have to use a convex combination of both samples. The estimator for the covariance function will look as follows
\begin{align*}
    \hat{c}_{\hat{\vartheta}, \lambda} := \hat{\vartheta} \hat{c}^{(1)}_\lambda + (1- \hat{\vartheta}) \hat{c}^{(2)}_\lambda,
\end{align*}
where
\begin{align*}
    \hat{c}^{(1)}_\lambda &:= \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \br{X_i - \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} X_j} \otimes \br{X_i - \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} X_j}\\
    \hat{c}^{(2)}_\lambda &:= \frac{1}{\gbr{\lambda (n-\gbr{n \hat{\vartheta}})}} \sum_{i=\gbr{n \hat{\vartheta}}+1}^{\gbr{n \hat{\vartheta}} + \gbr{\lambda (n-\gbr{n \hat{\vartheta}})}} \br{X_i - \frac{1}{\gbr{\lambda (n-\gbr{n \hat{\vartheta}})}} \sum_{j=\gbr{n \hat{\vartheta}}+1}^{\gbr{n \hat{\vartheta}} + \gbr{\lambda (n-\gbr{n \hat{\vartheta}})}} X_j} \\
    &\phantom{asdfasdfasdasdadsasassaadfaadsf} \otimes \br{X_i - \frac{1}{\gbr{\lambda (n-\gbr{n \hat{\vartheta}})}} \sum_{j=\gbr{n \hat{\vartheta}}+1}^{\gbr{n \hat{\vartheta}} + \gbr{\lambda (n-\gbr{n \hat{\vartheta}})}} X_j}
\end{align*}
and we will put $\hat{c}^{(i)}_\lambda := 0$ for $i=1,2$ if $\gbr{\lambda n} = 0$ (because then $\lambda \gbr{n \hat{\vartheta}} \leq \lambda n < 1$, i.e. $\gbr{\lambda \gbr{n \hat{\vartheta}}} = 0$.)
Moreover, define $$c_{\vartheta_0} := \vartheta_0 c^{(1)} + (1-\vartheta_0) c^{(2)} $$

%$$c := \vartheta_0 \E {\eta_0^{(1)} \otimes \eta_0^{(1)}} + (1-\vartheta_0) \E {\eta_0^{(2)} \otimes \eta_0^{(2)}} $$

The next theorem shows that the above estimator is $L^2$-consistent.
\begin{thm}
    Under assumption \ref{ass_4th} and $\vartheta_0 \in (\varepsilon, 1- \varepsilon)$, we have
    \begin{align*}
        \sup_{0 \leq \lambda \leq 1} \sqrt{\lambda} \norm{\hat{c}_{\hat{\vartheta}, \lambda} - c_{\vartheta_0}}_2 = O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}}.
    \end{align*}
\end{thm}

\begin{proof}
    We show that
    \begin{align*}
        \sup_{0 \leq \lambda \leq 1} \sqrt{\lambda} \norm{\hat{\vartheta} \hat{c}^{(1)}_\lambda - \vartheta_0 \E {\eta_0^{(1)} \otimes \eta_0^{(1)}}}_2 = O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}}.
    \end{align*}
    By similar arguments, one also shows the analogous result for $(1- \hat{\vartheta}) \hat{c}_\lambda^{(2)}$. First, we assume that $\lambda < \frac{1}{n}$, then $\gbr{\lambda n} = 0$, $\hat{c}^{(1)} = 0$ and 
    \begin{align*}
        \sqrt{\lambda} \norm{\hat{\vartheta} \hat{c}^{(1)}_\lambda - \vartheta_0 \E {\eta_0^{(1)} \otimes \eta_0^{(1)}}}_2 < \frac{\vartheta_0}{\sqrt{n}} \bigg| \E {\eta_0^{(1)} \otimes \eta_0^{(1)}} \bigg| = O_\p (n^{-1/2})
    \end{align*}
    uniformly in $\lambda$. Now, assume that $\frac{1}{n} \leq \lambda \leq 1$ and expand
    \begin{align}\label{disp:expansion}
        \hat{c}^{(1)}_\lambda = \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} X_i \otimes X_i - \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2 } \sum_{i,j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} X_i \otimes X_j
    \end{align}
    by a simple calculation. Considering the first term, we get
    \begin{align*}
        \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} X_i \otimes X_i &= \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}} \wedge \gbr{n \vartheta_0}} X_i \otimes X_i + \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=\gbr{\lambda \gbr{n \hat{\vartheta}}} \wedge \gbr{n \vartheta_0} + 1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} X_i \otimes X_i\\
        &= \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}} \wedge \gbr{n \vartheta_0}} \br{\eta_i^{(1)} \otimes \eta_i^{(1)} + \mu \otimes \eta_i^{(1)} + \eta_i^{(1)} \otimes \mu + \mu \otimes \mu} \\
        &\phantom{afdas}+ \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=\gbr{\lambda \gbr{n \hat{\vartheta}}} \wedge \gbr{n \vartheta_0} + 1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \br{\eta_i^{(2)} \otimes \eta_i^{(2)} + \tilde{\mu} \otimes \eta_i^{(2)} + \eta_i^{(2)} \otimes \tilde{\mu} + \tilde{\mu} \otimes \tilde{\mu}},
    \end{align*}
    where $\tilde{\mu} := \mu + \delta$. The second sum will be zero if $\gbr{\lambda \gbr{n \hat{\vartheta}}} \leq \gbr{n \vartheta_0}$. The second term in (\ref{disp:expansion}) can be rewritten as follows:
    \begin{align*}
        \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2 }& \sum_{i,j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} X_i \otimes X_j\\
        &\ppad= \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2 } \sum_{i,j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \br{\eta_i^{(1)} \otimes \eta_j^{(1)} + \mu \otimes \eta_j^{(1)} + \eta_i^{(1)} \otimes \mu + \mu \otimes \mu}\\
        &\pppad\ppad + \frac{\mathbbm{1} \cbr{\gbr{n \vartheta_0} \leq \gbr{\lambda \gbr{n \hat{\vartheta}}}}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2} \bigg[ \sum_{i=1}^{\gbr{n \vartheta_0}} \sum_{j= \gbr{n \vartheta_0}+1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \br{\eta_i^{(1)} \otimes \eta_j^{(2)} + \mu \otimes \eta_j^{(2)} + \eta_i^{(1)} \otimes \tilde{\mu} + \mu \otimes \tilde{\mu}}\\
        &\phantom{asdfasdfasdfasdfasdasdfsdfa} + \sum_{i= \gbr{n \vartheta_0}+1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{j=1}^{\gbr{n \vartheta_0}}  \br{\eta_i^{(2)} \otimes \eta_j^{(1)} +  \eta_i^{(2)} \otimes \mu +  \tilde{\mu} \otimes \eta_j^{(1)} + \tilde{\mu} \otimes \mu}\\
        &\phantom{asdfasdfasdfasdfaasdsdfsdfa} + \sum_{i,j= \gbr{n \vartheta_0}+1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \br{\eta_i^{(2)} \otimes \eta_j^{(2)} +  \eta_i^{(2)} \otimes \tilde{\mu} +  \tilde{\mu} \otimes \eta_j^{(2)} + \tilde{\mu} \otimes \tilde{\mu}} \bigg].
    \end{align*}
    Analogous but tedious calculations, combining with (\ref{disp:expansion}) lead to the result that if $\gbr{\lambda \gbr{n \hat{\vartheta}}} \leq \gbr{n \vartheta_0}$, we have
    \begin{align*}
        \hat{c}_\lambda = \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_i^{(1)} \otimes \eta_i^{(1)} - \frac{1}{ \gbr{\lambda \gbr{n \hat{\vartheta}}}^2} \sum_{i,j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_i^{(1)} \otimes \eta_j^{(1)}
    \end{align*}
    and
    \begin{align*}
        \hat{c}_\lambda &= \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{n \vartheta_0}} \eta_i^{(1)} \otimes \eta_i^{(1)} - \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2} \sum_{i,j=1}^{\gbr{n \vartheta_0}} \eta_i^{(1)} \otimes \eta_j^{(1)} + \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i= \gbr{n \vartheta_0} + 1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} (\eta_i^{(2)} + \delta) \otimes (\eta_i^{(2)} + \delta) \\
        &\ppad - \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2} \sum_{i=1}^{\gbr{n \vartheta_0}} \sum_{j=\gbr{n \vartheta_0} +1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_i^{(1)} \otimes (\eta_j^{(2)} + \delta) - \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2} \sum_{i=\gbr{n \vartheta_0} +1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{j=1}^{\gbr{n \vartheta_0}}  (\eta_i^{(2)} + \delta) \otimes \eta_j^{(1)}\\
        &\ppad \frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}^2} \sum_{i,j= \gbr{n \vartheta_0}}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} (\eta_i^{(2)} + \delta) \otimes (\eta_j^{(2)} + \delta)
    \end{align*}
    if $\gbr{\lambda \gbr{n \hat{\vartheta}}} \geq \gbr{n \vartheta_0}$. We start with the case $\gbr{\lambda \gbr{n \hat{\vartheta}}} \leq \gbr{n \vartheta_0}$, where we have
    \begin{align*}
        \sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \hat{\vartheta} \norm{\frac{1}{ \gbr{\lambda \gbr{n \hat{\vartheta}}}^2} \sum_{i,j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_i^{(1)} \otimes \eta_j^{(1)}}_2 &= \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{\lambda \hat{\vartheta}}{\gbr{\lambda \gbr{ n \hat{\vartheta}}}} \frac{1}{\sqrt{\lambda}} \norm{\frac{1}{ \sqrt{\gbr{\lambda \gbr{n \hat{\vartheta}}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_i^{(1)}}^2\\
        &\leq O_\p (n^{-1/2}) \br{\sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{ \sqrt{\gbr{\lambda n}}} \norm{ \sum_{i=1}^{\gbr{\lambda n}} \eta_i^{(1)}} }^2 = O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}}.
    \end{align*}
    We expanded the set over which we take the supremum and in the last step, we used (\ref{disp:aue_lemma_b1}).
    %a slight variation of Lemma B.1 from the online supplementary material of \cite{aue2}, which states that
    %\begin{align}\label{disp:aue_lemma_b1}
    %    \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\sqrt{\gbr{\lambda n}}} \norm{\sum_{i=1}^{\gbr{\lambda n}} \eta_i} = O_\p (\log^{1/\kappa} (n))
    %\end{align}
    %for $L^2(S \times \sqbr{0,1})$-valued random variables $\cbr{\eta_i}_{i \in \mathbb{Z}}$.
    Now, taking into account what we have just proved, we get
    \begin{align*}
        \sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \norm{\hat{\vartheta} \hat{c}_\lambda - \vartheta_0 \E{\eta_0^{(1)} \otimes \eta_0^{(1)}}}_2 &\leq \sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \norm{ \frac{\hat{\vartheta}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \br{\eta_i^{(1)} \otimes \eta_i^{(1)} - \E{\eta_0^{(1)} \otimes \eta_0^{(1)}}}}_2\\
        &\pppad\pppad + |\hat{\vartheta} - \vartheta_0 | \E{\eta_0^{(1)} \otimes \eta_0^{(1)}} + O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}}\\
        &\leq O_\p (n^{-1/2}) \sup_{\frac{1}{n} \leq \lambda \leq 1} 
        %\frac{1}{\sqrt{n}} \frac{\lambda n \hat{\vartheta}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \frac{\sqrt{\gbr{\lambda n}}}{ \sqrt{\lambda n}} 
        \frac{1}{\sqrt{\gbr{\lambda n}}} \norm{ \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \br{\eta_i^{(1)} \otimes \eta_i^{(1)} - \E{\eta_0^{(1)} \otimes \eta_0^{(1)}}} }_2\\
        &\pppad\pppad + O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}}\\
        &\leq O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}},
    \end{align*}
    where we again used a variation of (\ref{disp:aue_lemma_b1}), this time for $L^2 ((S \times \sqbr{0,1})^2)$-valued random variables, which is also of the order $O_\p (\log^{1/\kappa} (n))$.

    It remains to show that we reach the same conclusion when $\gbr{\lambda \gbr{n \hat{\vartheta}}} \geq \gbr{n \vartheta_0}$. In this case, we claim that
    \begin{align*}
        \sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \norm{\hat{\vartheta} \hat{c}_\lambda - \vartheta_0 \E{\eta_0^{(1)} \otimes \eta_0^{(1)}} }_2 &= \sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \norm{\frac{\hat{\vartheta}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{n \vartheta_0}} \eta_i^{(1)} \otimes \eta_i^{(1)} - \vartheta_0 \E{\eta_0^{(1)} \otimes \eta_0^{(1)}} }_2\\
        &\pppad + O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}}
    \end{align*}
    and for this we show that
    \begin{enumerate}
        \item $\displaystyle \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}} } \sum_{i=1}^{\gbr{n \vartheta_0}} \eta_i^{(1)} } = O_\p (n^{-1/2})$,
        
        \item $\displaystyle \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=\gbr{n \vartheta_0} + 1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} (\eta_i^{(2)} + \delta) } = O_\p \br{\frac{\log^{1/\kappa} (n)}{\sqrt{n}}}$,
        
        \item $\displaystyle \sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \hat{\vartheta} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i= \gbr{n \vartheta_0} +1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} (\eta_i^{(2)} + \delta) }^2 = O_\p \br{\frac{\log^{2/\kappa} (n)}{\sqrt{n}}}$,
        
        \item $\displaystyle \sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \hat{\vartheta} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=\gbr{n \vartheta_0} + 1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}}  (\eta_i^{(2)} + \delta) \otimes (\eta_i^{(2)} + \delta)} = O_\p \br{\frac{\log^{1/\kappa} (n)}{\sqrt{n}}}$.
    \end{enumerate}

    The first equality follows from
    \begin{align*}
        \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}} } \sum_{i=1}^{\gbr{n \vartheta_0}} \eta_i^{(1)} } \leq \frac{1}{\sqrt{\gbr{n \vartheta_0}}} \norm{\frac{1}{\sqrt{\gbr{n \vartheta_0}}} \sum_{i=1}^{\gbr{n \vartheta_0}} \eta_i^{(1)} } = O_\p (n^{1/2}),
    \end{align*}
    because of the central limit theorem in Hilbert spaces and $\gbr{n \vartheta_0} \leq \gbr{\lambda \gbr{n \hat{\vartheta}}}$. For the second equality, recall that by Proposition \ref{prop:changepoint_conv_rate}, we have $\hat{\vartheta} = \vartheta_0 + o_\p (n^{-1/2})$. Using the rate in (\ref{disp:aue_lemma_b1}) and again $\gbr{n \vartheta_0} \leq \gbr{\lambda \gbr{n \hat{\vartheta}}}$, we find that
    \begin{align*}
        \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=\gbr{n \vartheta_0} + 1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} (\eta_i^{(2)} + \delta) } & \leq \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\sqrt{\gbr{n \vartheta_0}}} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_i^{(2)} }\\
        &\pppad + \frac{1}{\sqrt{\gbr{n \vartheta_0}}} \norm{\frac{1}{\sqrt{\gbr{n \vartheta_0}}} \sum_{i=1}^{\gbr{n \vartheta_0}} \eta_i^{(2)} } + \frac{\gbr{\lambda \gbr{n \hat{\vartheta}}} - \gbr{n \vartheta_0}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \norm{\delta}\\
        &\leq O_\p (n^{-1/2}) \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\frac{1}{\gbr{\lambda n}} \sum_{i=1}^{\gbr{\lambda n}} \eta_i^{(2)} } + O_\p (n^{-1/2}) \frac{\gbr{n \hat{\vartheta}} - \gbr{n \vartheta_0}}{\gbr{n \vartheta_0}} \norm{\delta}\\
        &= O_\p \br{\frac{\log^{1/\kappa} (n)}{\sqrt{n}}}.
    \end{align*}

    Combining the calculations above, one easily concludes the third assertion. For the fourth equality, we have again by a version of (\ref{disp:aue_lemma_b1}) for $L^2( (S \times \sqbr{0,1})^2 )$-valued random variables and the fact that $\gbr{n \vartheta_0} \leq \gbr{\lambda \gbr{n \hat{\vartheta}}}$ that
    \begin{align*}
        &\sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \hat{\vartheta} \norm{\frac{1}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=\gbr{n \vartheta_0} +1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} (\eta_i^{(2)} + \delta ) \otimes (\eta_i^{(2)} + \delta ) }_2\\
        &\pppad\leq \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\sqrt{\gbr{n \vartheta}}} \norm{\frac{1}{\sqrt{\gbr{\lambda \gbr{n \hat{\vartheta}}}}} \sum_{i=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}}  \tilde{\eta}^\otimes_i  }_2 + o_\p (n^{-1/2}) \E{(\eta_0^{(2)} + \delta) \otimes (\eta_0^{(2)} + \delta)}\\
        &\pppad= O_\p \br{\frac{\log^{1/\kappa} (n)}{\sqrt{n}}},
    \end{align*}
    where $\tilde{\eta}^\otimes_i := (\eta_i^{(2)} + \delta) \otimes (\eta_i^{(2)} + \delta) - \E{(\eta_0^{(2)} + \delta) \otimes (\eta_0^{(2)} + \delta)}$. Lastly, note that $\frac{\gbr{n \vartheta_0}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} = 1 + o_\p (n^{-1/2})$, because
    $$1 + o_\p (n^{-1/2}) = \frac{\gbr{\lambda \gbr{n \vartheta_0}}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \leq \frac{\gbr{n \vartheta_0}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \leq \frac{\gbr{\lambda \gbr{n \hat{\vartheta}}}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} = 1$$ and therefore, we have
    \begin{align*}
        &\sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{\lambda} \norm{\frac{\hat{\vartheta}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \sum_{i=1}^{\gbr{n \vartheta_0}} \eta_i^{(1)} \otimes \eta_i^{(1)} - \vartheta_0 \E{\eta_0^{(1)} \otimes \eta_0^{(1)}} }_2\\
        &\pppad \leq \frac{1}{\sqrt{\gbr{n \vartheta_0}}} \norm{ \frac{1}{\sqrt{\gbr{n \vartheta_0}}} \sum_{i=1}^{\gbr{n \vartheta_0}} \br{\eta_i^{(1)} \otimes \eta_i^{(1)} - \E{\eta_0^{(1)} \otimes \eta_0^{(1)}}} }_2 + \sup_{\frac{1}{n} \leq \lambda \leq 1} \bigg| \frac{\gbr{n \vartheta_0}}{\gbr{\lambda \gbr{n \hat{\vartheta}}}}\hat{\vartheta} - \vartheta_0 \bigg| \E{\eta_0^{(1)} \otimes \eta_0^{(1)}}\\
        &\pppad = O_\p (n^{-1/2}) + o_\p ( n^{-1/2}) = O_\p (n^{-1/2})
    \end{align*}
    and the proof is complete.
\end{proof}

Next, we need to consider distances between the eigenfunctions of the operator corresponding to the kernel $\hat{c}_{\hat{\vartheta}, \lambda}$ and the eigenfunctions corresponding to $c_{\vartheta_0}$. We will denote the former by $\hat{w}_{1,\lambda}, \hat{w}_{2, \lambda}, ...$ with eigenvalues $\hat{\tau}_1, \hat{\tau}_2, ...$ and the latter by $w_1, w_2, ...$ with eigenvalues $\tau_1, \tau_2, ...$


\begin{prop}
    Suppose assumptions \ref{ass_4th} and \ref{eigvals_order} hold. If further $\vartheta_0 \in \br{\varepsilon, 1-\varepsilon}$, then for any $j \leq d$, we have
    \begin{align*}
        \sup_{0 \leq \lambda \leq 1} \norm{\lambda (\hat{c}_{j,\lambda} \hat{w}_{j,\lambda} - w_j) - \frac{1}{\sqrt{n}} \sum_{i \neq j} \frac{w_i}{\tau_j - \tau_i}  \innpr{\hat{Z}_{n, \lambda}, w_j \otimes w_i}_2  } = O_\p \br{\frac{\log^{4/\kappa} (n)}{n}},
    \end{align*}
    where $\hat{c}_{j \lambda} = \mathrm{sign} \innpr{\hat{w}_{j, \lambda}, w_j}$ and $$\hat{Z}_{n, \lambda} := \frac{1}{\sqrt{n}} \br{ \sum_{i=1}^{\gbr{\lambda \gbr{n \vartheta_0}}} (\eta_i^{(1)} \otimes \eta_i^{(1)} - c^{(1)}) + \sum_{i=\gbr{n \vartheta_0}+1}^{\gbr{n \vartheta_0} + \gbr{\lambda (n - \gbr{n \vartheta_0})}} (\eta_i^{(2)} \otimes \eta_i^{(2)} - c^{(2)})  }$$
\end{prop}


\begin{proof}
    Similar to the proof of Proposition 2.1 in \cite{aue}.
\end{proof}


We define the test statistic
\begin{align*}
    D_n (s,t,\lambda, \vartheta) := \frac{1}{\gbr{n \vartheta}} \sum_{i=1}^{\gbr{\lambda \gbr{n \vartheta}}} X_i (s,t) - \frac{1}{n - \gbr{n \vartheta}} \sum_{i= \gbr{n \vartheta} +1}^{\gbr{n \vartheta} + \gbr{\lambda (n - \gbr{n \vartheta})}} X_i(s,t)
\end{align*}

\begin{thm}
    Let
    \begin{align*}
        \sigma_{cp}^2 := &2\sum_{i\in \mathbb{Z}} \bigg( \vartheta_0 \sum_{s_1,...,s_4 \in S} \int \cov \br{ \eta_0^{(1)} (t_1, s_1) \eta_0^{(1)} (t_2, s_2) , \eta_i^{(1)} (t_3, s_3) \eta_i^{(1)} (t_4, s_4)} f((t_1, s_1), (t_2, s_2)) f((t_3, s_3), (t_4, s_4)) \mathrm{d} (t_1, ..., t_4) \\
        &- 2 \sum_{s_1, s_2, s_3 \in S} \int \cov \br{ \eta_0^{(1)} (t_1, s_1) \eta_0^{(1)} (t_2, s_2)  , \eta_i^{(1)} (t_3, s_3)  } f((t_1, s_1), (t_2, s_2)) w(t_3, s_3) \mathrm{d} (t_1, t_2, t_3)\\
        &+ \frac{1}{\vartheta_0} \sum_{s_1, s_2 \in S} \int \cov \br{\eta_0^{(1)} (t_1, s_1), \eta_i^{(1)} (t_2, s_2) } w(t_1, s_1) w(t_2, s_2) \mathrm{d} (t_1, t_2) \\
        &+  (1- \vartheta_0) \negthickspace \negthickspace \sum_{s_1,...,s_4 \in S} \int \cov \br{ \eta_0^{(2)} (t_1, s_1) \eta_0^{(2)} (t_2, s_2) , \eta_i^{(2)} (t_3, s_3) \eta_i^{(2)} (t_4, s_4)} f((t_1, s_1), (t_2, s_2)) f((t_3, s_3), (t_4, s_4)) \mathrm{d} (t_1, ..., t_4) \\
        &-2 \sum_{s_1, s_2, s_3 \in S} \int \cov \br{ \eta_0^{(2)} (t_1, s_1) \eta_0^{(2)} (t_2, s_2)  , \eta_i^{(2)} (t_3, s_3)  } f((t_1, s_1), (t_2, s_2)) w(t_3, s_3) \mathrm{d} (t_1, t_2, t_3)\\
        &+ \frac{1}{1-\vartheta_0}  \sum_{s_1, s_2 \in S} \int \cov \br{\eta_0^{(1)} (t_1, s_1), \eta_i^{(1)} (t_2, s_2) } w(t_1, s_1) w(t_2, s_2) \mathrm{d} (t_1, t_2) \bigg)
    \end{align*}
    and
    \begin{align*}
        w(s_1,t_1) := \sum_{k=1}^d \innpr{\delta, w_k} v_k (s_1, t_1) \pppad f((s_1, t_1), (s_2, t_2)) := \sum_{k=1}^d \innpr{\delta, w_k} w_k (s_1, t_1) \sum_{j \neq k} \frac{\innpr{\delta, w_j}}{\lambda_k - \lambda_j} w_j (s_2, t_2).
    \end{align*}
    If assumption \ref{ass_4th} is satisfied, $\norm{\delta}^2 > 0$ and $\vartheta_0 \in (\varepsilon, 1- \varepsilon)$, then the following statements are true.
    \begin{enumerate}
        \item As $n \to \infty$, $$\sqrt{n} \sum_{k=1}^d \br{\innpr{D_n (\lambda, \vartheta_0), \hat{w}_{k, \lambda}}^2 - \innpr{\delta, w_k}^2} \convproc \sigma_{cp} \cbr{\lambda \mathbb{B}(\lambda)}_{\lambda \in \sqbr{0,1}}.$$
        %%
        \item Replacing $\vartheta_0$ by $\hat{\vartheta}$ gives the same result, i.e. as $n \to \infty$ $$\sqrt{n} \sum_{k=1}^d \br{\innpr{D_n (\lambda, \hat{\vartheta}), \hat{w}_{k, \lambda}}^2 - \innpr{\delta, w_k}^2} \convproc \sigma_{cp} \cbr{\lambda \mathbb{B}(\lambda)}_{\lambda \in \sqbr{0,1}}.$$
    \end{enumerate}
\end{thm}

\begin{proof}
    \begin{enumerate}
        \item We have
            \begin{align*}
                \sqrt{n} \sum_{k=1}^d \br{\innpr{D_n (\lambda, \vartheta_0), \hat{w}_{k,\lambda}}^2 - \lambda^2 \innpr{\delta, w_k}^2} &= \frac{2 \lambda}{\sqrt{n}} \sum_{i=1}^{\gbr{\lambda \gbr{n \vartheta_0}}} \innpr{\eta_i^{(1)} \otimes \eta_i^{(1)} - c^{(1)}, f}_2\\
                &\pppad + \frac{2 \lambda}{\sqrt{n}} \sum_{i=\gbr{n \vartheta_0}+1}^{\gbr{n \vartheta_0} + \gbr{\lambda (n - \gbr{n \vartheta_0})}} \innpr{\eta_i^{(2)} \otimes \eta_i^{(2)} - c^{(2)}, f}_2 \\
                &\pppad - \frac{2 \lambda \sqrt{n}}{\gbr{n \vartheta_0}} \sum_{i=1}^{\gbr{\lambda \gbr{n \vartheta_0}}} \innpr{\eta_i^{(1)}, w}\\
                &\pppad - \frac{2 \lambda \sqrt{n}}{n - \gbr{n \vartheta_0}} \sum_{i=\gbr{n \vartheta_0} +1}^{\gbr{n \vartheta_0} + \gbr{\lambda (n - \gbr{n \vartheta_0})}} \innpr{\eta_i^{(2)}, w} + o_\p (1)\\
                &= 2 \lambda \br{\tilde{Z}_n^{(1)} \br{\frac{\lambda \gbr{n \vartheta_0}}{n}} + \tilde{Z}_n^{(2)} \br{\frac{\gbr{n \vartheta_0} + \gbr{\lambda (n - \gbr{n \vartheta_0})}}{n}} - \tilde{Z}_n^{(2)} \br{\vartheta_0} },
            \end{align*}
            where for $k=1,2$
            \begin{align*}
                \tilde{Z}_n^{(k)} (\lambda) = \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{\lambda n}} \br{\innpr{\eta_i^{(k)} \otimes \eta_i^{(k)}, \xi_k}_2 + \innpr{\eta_i^{(k)}, \zeta_k}}  
            \end{align*}
            with $\xi_1 = \xi_2 = f$, $\zeta_1 = - \frac{1}{\vartheta_0} w$ and $\zeta_2 = - \frac{1}{1-\vartheta_0} w$. Now by Lemma \ref{general_lemma_b1}, we obtain
            \begin{align*}
                \sqrt{n} \sum_{k=1}^d \br{\innpr{D_n (\lambda, \vartheta_0), \hat{w}_{k,\lambda}}^2 - \lambda^2 \innpr{\delta, w_k}^2} \convproc 2 \lambda \mathbb{Z}^{(1)} \br{\lambda \vartheta_0} + 2 \lambda \br{\mathbb{Z}^{(2)} \br{\vartheta_0 + \lambda (1- \vartheta_0)} - \mathbb{Z}^{(2)} \br{\vartheta_0}},
            \end{align*} 
            where $\mathbb{Z}^{(1)} (\lambda) := \tilde{\Sigma}_{11} \mathbb{B}_1 (\lambda) + \tilde{\Sigma}_{12} \mathbb{B}_2(\lambda)$ and $\mathbb{Z}^{(2)} (\lambda) := \tilde{\Sigma}_{21} \mathbb{B}_1 + \tilde{\Sigma}_{22} \mathbb{B}_2$.
            $\tilde{\Sigma}_{ij}$ denotes the $ij$-th entry of the matrix $\Sigma^{1/2}$ and $\Sigma$ is the matrix with entries as given in the previously mentioned Lemma. Inspecting the covariance structure of the limiting process, we see that
            \begin{align*}
                \cov &\br{\mathbb{Z}^{(1)} (\lambda_1 \vartheta_0) + \mathbb{Z}^{(2)} (\vartheta_0 + \lambda_1 (1-\vartheta_0)) - \mathbb{Z}^{(2)} (\vartheta_0), \mathbb{Z}^{(1)} (\lambda_2 \vartheta_0) + \mathbb{Z}^{(2)} (\vartheta_0 + \lambda_2 (1-\vartheta_0)) - \mathbb{Z}^{(2)} (\vartheta_0)}\\
                &= (\lambda_1 \wedge \lambda_2)(\Sigma_{11} \vartheta_0 + \Sigma_{22} (1-\vartheta_0))
            \end{align*}
            and hence the first claim follows. 
            %%%
            \item \blue{For the second assertion, we show that $$\sup_{0 \leq \lambda \leq 1} (\innpr{D_n (\lambda, \vartheta_0), \hat{w}_{k,\lambda}}^2 - \innpr{D_n (\lambda, \hat{\vartheta}), \hat{w}_{k, \lambda}}^2) = o_\p (n^{-1/2}).$$ We have by part 1 and 2 of Lemma \ref{lem:approx_for_cp_in_summation}
            \begin{align*}
                \sup_{0 \leq \lambda \leq 1}& (\innpr{D_n (\lambda, \hat{\vartheta}), \hat{w}_{k,\lambda}}^2 - \innpr{D_n (\lambda, \vartheta_0), \hat{w}_{k,\lambda}}^2)\\
                &=\sup_{0 \leq \lambda \leq 1} \br{\innpr{\tilde{D}_n (\lambda, \hat{\vartheta}), \hat{w}_{k, \lambda}}^2 - \innpr{\tilde{D}_n (\lambda, \vartheta_0), \hat{w}_{k, \lambda}}^2 + 2 \lambda \innpr{\delta, \hat{w}_{k, \lambda}} \innpr{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0), \hat{w}_{k, \lambda}}}\\
                &=\sup_{0 \leq \lambda \leq 1} \bigg( \innpr{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0), \hat{w}_{k,\lambda}}^2 + 2 \innpr{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0), \hat{w}_{k, \lambda}} \innpr{\tilde{D}_n (\lambda, \vartheta_0), \hat{w}_{k, \lambda}}\\
                &\pppad\pppad\pppad + 2 \lambda \innpr{\delta, \hat{w}_{k, \lambda}} \innpr{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0), \hat{w}_{k, \lambda}} \bigg)\\
                &\leq \sup_{0 \leq \lambda \leq 1} \norm{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0)}^2  \norm{\hat{w}_{k, \lambda}}^2 + 2\sup_{0 \leq \lambda \leq 1} \norm{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0)}^2 \norm{\tilde{D}_n (\lambda, \vartheta_0)} \norm{\hat{w}_{k,\lambda}}^2\\
                &\pppad\pppad\pppad + 2 \sup_{0 \leq \lambda \leq 1} \norm{\delta} \norm{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0)} \norm{\hat{w}_{k, \lambda}}^2\\
                &= o_\p (n^{-1/2})
            \end{align*}}
    \end{enumerate}
\end{proof}



Now, we can formulate the test as follows: Reject $H_0$ if
\begin{align}\label{disp:cp_mean_testrule}
    \sum_{k=1}^d \innpr{D_n(1, \hat{\vartheta}), \hat{w}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{Y}}_n,
\end{align}
where $$\hat{\mathbb{Y}}_n := \br{\int_0^1 \br{\sum_{k=1}^d  \innpr{ D_n (\lambda, \hat{\vartheta}) , \hat{w}_{k, \lambda} }^2 - \lambda^2 \innpr{D_n (1, \hat{\vartheta}), \hat{w}_k}^2  }^2 \mathrm{d} \nu (\lambda) }^{1/2},$$ for some probability measure $\nu$ on $(0,1)$.

The next theorem is the consistency result of this decision rule. The proof goes the same way as in the previous chapters and is therefore omitted.
\begin{thm}
    We have
    \begin{align*}
        \lim_{n \to \infty} \P{\sum_{k=1}^d \innpr{D_n(1, \hat{\vartheta}), \hat{w}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{Y}}_n} = \begin{cases}
            0,& \text{if } \norm{\delta}^2 < \Delta,\\
            1,& \text{if } \norm{\delta}^2 > \Delta
        \end{cases}
    \end{align*}
    and if $\norm{\delta}^2 = \Delta$ and $\sigma_{cp}^2 > 0$ then
    \begin{align*}
        \lim_{n \to \infty} \P{\sum_{k=1}^d \innpr{D_n(1, \hat{\vartheta}), \hat{w}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{Y}}_n} \leq \alpha.
    \end{align*}
\end{thm}


\begin{rem}
    Again, we can test the hypotheses
    \begin{center}
        $H_0: \sum_{k=1}^d \innpr{\delta, w_k}^2 \leq \Delta$ vs. $H_1: \sum_{k=1}^d \innpr{\delta, w_k}^2 > \Delta$
    \end{center}
    and obtain the result
    \begin{align*}
        \lim_{n \to \infty} \P{\sum_{k=1}^d \innpr{D_n(1, \hat{\vartheta}), \hat{w}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{Y}}_n} = \begin{cases}
            0,& \text{if } \sum_{k=1}^d \innpr{\delta, w_k}^2 < \Delta,\\
            \alpha,& \text{if } \sum_{k=1}^d \innpr{\delta, w_k}^2 = \Delta,\\
            1,& \text{if } \sum_{k=1}^d \innpr{\delta, w_k}^2 > \Delta
        \end{cases}
    \end{align*}
    for the decision rule proposed in (\ref{disp:cp_mean_testrule}).
\end{rem}





==> proj_onesample.tex <==
Define for $s_1, s_2 \in S$ and $t_1, t_2 \in \sqbr{0,1}$
\begin{align*}
    v(s_1,t_1) := \sum_{k=1}^d \innpr{\mu, v_k} v_k (s_1, t_1), \pppad f((s_1, t_1), (s_2, t_2)) := \sum_{k=1}^d \innpr{\mu, v_k} v_k (s_1, t_1) \sum_{j \neq k} \frac{\innpr{\mu, v_j}}{\lambda_k - \lambda_j} v_j (s_2, t_2).
\end{align*}

\begin{thm}\label{projconv}
    Let $\cbr{X_j}_{j \in \mathbb{Z}}$ be a sequence of random functions, which satisfies assumption \ref{ass_4th}. Then
    \begin{align*}
        \sqrt{n} \sum_{k=1}^d \br{\innpr{\overline{X}_{\gbr{n \lambda}}, \hat{v}_{k, \lambda}}^2 - \lambda^2 \innpr{\mu, v_k}^2 } \convproc \sigma \cbr{\lambda \mathbb{B} (\lambda)}_{\lambda \in \sqbr{0,1}},
    \end{align*}
    where $\cbr{\mathbb{B} (\lambda)}$ is a standard Brownian motion and
    \begin{align*}
        &\sigma^2 := 4 \sum_{h \in \mathbb{Z}} \bigg( \sum_{s_1, s_2 \in S} \int \negthickspace \int \mathrm{Cov} (\eta_0 (s_1, t_1), \eta_h (s_2, t_2)) v (s_1, t_1) v (s_2, t_2)\mathrm{d}t_1 \mathrm{d}t_2\\
         &\pad + 2 \sum_{s_1, s_2, s_3 \in S} \int \negthickspace \int \negthickspace \int \negthickspace \mathrm{Cov} (\eta_0 (s_1, t_1), \eta_h (s_2, t_2) \eta_h (s_3, t_3)) v(s_1, t_1) f((s_2, t_2), (s_3, t_3)) \mathrm{d}t_1 \mathrm{d}t_2 \mathrm{d}t_3\\ 
         &\pad + \sum_{s_1, s_2, s_3, s_4 \in S} \int \negthickspace \int \negthickspace \int \negthickspace \int \mathrm{Cov} (\eta_0 (s_1, t_1) \eta_0 (s_2, t_2), \eta_h (s_3, t_3) \eta_h (s_4, t_4)) f ((s_1, t_1), (s_2, t_2)) f ((s_3, t_3), (s_4, t_4)) \mathrm{d}t_1 \mathrm{d}t_2 \mathrm{d}t_3 \mathrm{d}t_4 \bigg).
    \end{align*}
\end{thm}


Lastly, we need the following Proposition, which can be found by generalizing Proposition 2.1 in \cite{aue} to eigenvectors of a covariance operator corresponding to random functions defined on $S \times \sqbr{0,1}$.

\begin{prop}\label{general_prop_21}
    Assume $\cbr{X_j}_{j \in \mathbb{Z}}$ satisfies assumption \ref{ass_4th}. Furthermore, suppose that the eigenvalues of its covariance operator satisfies assumption \ref{eigvals_order}. Let $\hat{c}_{j,\lambda} = \mathrm{sign}\innpr{\hat{v}_{j, \lambda} , v_j}$. Then for any $j \leq d$, we have
    \begin{align*}
        \sup_{0 \leq \lambda \leq 1} \norm{\lambda \br{\hat{c}_{j,\lambda} \hat{v}_{j, \lambda} - v_j} - \frac{1}{\sqrt{n}} \sum_{i \neq j} \frac{v_i}{\lambda_j - \lambda_i}  \innpr{\hat{Z}_{n, \lambda}, v_j \otimes v_i }_2 } = O_\p \br{\frac{\log^{\kappa} (n)}{n}},
    \end{align*}
    and
    \begin{align*}
        \sup_{0 \leq \lambda \leq 1} \sqrt{\lambda} \norm{\hat{v}_{j, \lambda} - v_j} = O_\p \br{\frac{\log^{1/\kappa} (n)}{\sqrt{n}}}
    \end{align*}
    for some $\kappa > 0$, where
    \begin{align*}
        \hat{Z}_{n, \lambda} \br{(s_1, t_1), (s_2, t_2)} := \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{n \lambda}} \br{ (X_i(s_1, t_1) - \mu (s_1, t_1)) (X_i (s_2, t_2) - \mu(s_2, t_2))  - c\br{(s_1, t_1), (s_2, t_2)}}.
    \end{align*}
\end{prop}

\begin{proof}[Proof of Theorem \ref{projconv}]
    Define for $s \in S$ and $t \in \sqbr{0,1}$ 
    \begin{align*}
        \tilde{X}_{\gbr{n \lambda}} (s,t) := \frac{1}{n} \sum_{i=1}^{\gbr{n \lambda}} (X_i (s,t) - \mu(s,t)),
    \end{align*}
    then for $k=1,...,d$ and $\lambda \in \sqbr{0,1}$ we have
    \begin{align*}
        \innpr{\overline{X}_{\gbr{n \lambda}}, \hat{v}_{k, \lambda}}^2 - \lambda^2 \innpr{\mu, v_k}^2 &= \innpr{\tilde{X}_{\gbr{n \lambda}}, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda} }^2 + 2 \lambda \innpr{\tilde{X}_{\gbr{n\lambda}}, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda} } \innpr{\mu, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda}}\\
        &\pppad\pppad + \lambda^2 \innpr{\mu, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda}}^2 - \lambda^2 \innpr{\mu, v_k}^2 \\
        &=I_{1,k} (\lambda) + I_{2,k} (\lambda) + I_{3,k} (\lambda),
    \end{align*}
    where
    \begin{align*}
        I_{1,k} (\lambda) &:= \innpr{\tilde{X}_{\gbr{n \lambda}}, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda} }^2,\\
        I_{2,k} (\lambda) &:= 2 \lambda \innpr{\tilde{X}_{\gbr{n\lambda}}, \hat{c}_{k, \lambda}\hat{v}_{k, \lambda} } \innpr{\mu, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda}},\\
        I_{3,k} (\lambda) &:= \lambda^2 \innpr{\mu, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda}}^2 - \lambda^2 \innpr{\mu, v_k}^2.
    \end{align*}
    By Theorem \ref{generalberkes} $\norm{\sqrt{n} \tilde{X}_{\gbr{n \lambda}}}$ is bounded and therefore by the Cauchy-Schwarz inequality, we obtain
    \begin{align*}
        \sqrt{n} I_{1,k} (\lambda) &\leq \frac{1}{\sqrt{n}} \norm{\sqrt{n} \tilde{X}_{\gbr{n \lambda}}}^2 \cdot \norm{\hat{v}_{k,\lambda} }^2 = o_\p (1).
    \end{align*}
    Moving to the second term, we get
    \begin{align*}
        \sqrt{n} I_{2,k} (\lambda) &= 2 \sqrt{n} \lambda \bigg(\innpr{\tilde{X}_{\gbr{n \lambda}}, \hat{c}_{k, \lambda} \hat{v}_{k,\lambda} - v_k} \innpr{\mu, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda} - v_k } + \innpr{\tilde{X}_{\gbr{n \lambda}}, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda} - v_k } \innpr{\mu, v_k}\\
        &\pppad\pppad\pppad + \innpr{\tilde{X}_{\gbr{n \lambda}}, v_k } \innpr{\mu, \hat{c}_{k, \lambda} \hat{v}_{k, \lambda} - v_k} + \innpr{\tilde{X}_{\gbr{n \lambda}}, v_k } \innpr{\mu, v_k} \bigg)\\
        &= 2\lambda \innpr{\sqrt{n} \tilde{X}_{\gbr{n \lambda}}, v_k } \innpr{\mu, v_k} + o_\p (1)
    \end{align*}
    again by Theorem \ref{generalberkes} and the second part of Proposition \ref{general_prop_21}. The third term yields
    \begin{align*}
        \sqrt{n} I_{3,k} (\lambda) &=  \innpr{\mu, \lambda \br{\hat{c}_{k, \lambda} \hat{v}_{k, \lambda} - v_k} }^2  + 2\lambda  \innpr{\mu, \lambda \br{\hat{c}_{k, \lambda} \hat{v}_{k, \lambda} - v_k}} \innpr{\mu, v_k}\\
        &= 2 \lambda \innpr{\mu, v_k} \innpr{\mu, \frac{1}{\sqrt{n}} \sum_{i \neq k} \frac{v_i}{\lambda_k - \lambda_i} \innpr{\hat{Z}_{n, \lambda}, v_k \otimes v_i}_2 } + o_\p (1),
    \end{align*}
    which finally leads to
    \begin{align*}
        &\sqrt{n} \sum_{k=1}^d\br{\innpr{\overline{X}_{\gbr{n \lambda}}, \hat{v}_{k, \lambda}}^2 - \lambda^2 \innpr{\mu, v_k}^2}\\
        &\pppad\pppad  =  2 \lambda \sqrt{n} \sum_{k=1}^d \innpr{\sqrt{n} \tilde{X}_{\gbr{n \lambda}}, v_k } \innpr{\mu, v_k} + 2 \lambda \sqrt{n} \sum_{k=1}^d \innpr{\mu, v_k} \innpr{\mu, \frac{1}{\sqrt{n}} \sum_{i \neq k} \frac{v_i}{\lambda_k - \lambda_i} \innpr{\hat{Z}_{n, \lambda}, v_k \otimes v_i}_2 } + o_\p (1) \\
        & \pppad\pppad = 2 \lambda \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{n\lambda}} \innpr{\eta_i, v} + 2 \lambda \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{n\lambda}} \innpr{\eta_i \otimes \eta_i - c, f}_2 + o_\p (1),
    \end{align*}
    where $\eta_i = X_i - \mu$. Next apply Lemma \ref{general_lemma_b1} with $\zeta_1 = v$, $\xi_1 = f$ and $\zeta_2 \equiv 0$, $\xi_2 \equiv 0$ to obtain
    \begin{align*}
        \cbr{\sqrt{n} \sum_{k=1}^d\br{\innpr{\overline{X}_{\gbr{n \lambda}}, \hat{v}_{k, \lambda }}^2 - \lambda^2 \innpr{\mu, v_k}^2}}_{\lambda \in \sqbr{0,1}} \convproc \cbr{2 \lambda \br{\mathbb{Z}_1 (\lambda) + \mathbb{Z}_2 (\lambda)}}_{\lambda \in \sqbr{0,1}},
    \end{align*}
    where
    \begin{align*}
        \mathbb{Z}_1 (\lambda) := \tilde{\Xi}_{11} \mathbb{B}_1 (\lambda) + \tilde{\Xi}_{12} \mathbb{B}_2 (\lambda) \ppad \text{ and } \ppad \mathbb{Z}_2 (\lambda) := \tilde{\Xi}_{21} \mathbb{B}_1 (\lambda) + \tilde{\Xi}_{22} \mathbb{B}_2 (\lambda),
    \end{align*}
    $\tilde{\Xi}_{ij}$ are the entries of $\Xi^{1/2}$ and $\Xi$ is defined by the entries
    \begin{align*}
        \Xi_{11} &:= \sum_{h \in \mathbb{Z}} \cov \br{\innpr{\eta_0 \otimes \eta_0, f}_2, \innpr{\eta_h \otimes \eta_h, f}_2},\\
        \Xi_{21} = \Xi_{12} &:= \sum_{h \in \mathbb{Z}} \cov \br{\innpr{\eta_0 \otimes \eta_0, f}_2, \innpr{\eta_h, v}},\\
        \Xi_{22} &:= \sum_{h \in \mathbb{Z}} \cov \br{\innpr{\eta_0, v}, \innpr{\eta_h, v}}.
    \end{align*}
    Since
    \begin{align*}
        \mathrm{Cov} \br{\lambda_1 \br{\mathbb{Z}_1 (\lambda_1) + \mathbb{Z}_2 (\lambda_1)},  \lambda_2 \br{\mathbb{Z}_1 (\lambda_2) + \mathbb{Z}_2 (\lambda_2)}} = \lambda_1 \lambda_2 (\lambda_1 \wedge \lambda_2) \br{\Xi_{11} + 2 \Xi_{12} + \Xi_{22}}
    \end{align*}
    we obtain the stated result.
\end{proof}

To establish the decision rule for the problem
\begin{center}
    $H_0: \norm{\mu}^2 \leq \Delta$ vs. $H_1 : \norm{\mu}^2 > \Delta$ 
\end{center}
we need to define the following quantities:
\begin{align*}
    \hat{\mathbb{V}}_n := \br{\int_0^1 \br{\sum_{k=1}^d \br{\innpr{\overline{X}_{\gbr{n\lambda}} , \hat{v}_{k, \lambda}}^2 - \lambda^2 \innpr{\overline{X}_n, \hat{v}_{k}}^2 } }^2 \mathrm{d}\nu (\lambda)}^{1/2},
\end{align*}
where $\nu$ denotes a probability measure on $(0,1)$. Then the rule will be as follows: Reject $H_0$ if
\begin{align}\label{decision_rule_proj_onesample}
    \sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_{k}}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n.
\end{align}
$q_{1-\alpha} (\mathbb{W})$ is the $(1-\alpha)$-quantile of the random variable defined in (\ref{disp:random_variable_w}).

% The next theorem shows that the rule defined in (\ref{decision_rule_proj_onesample}) defines a consistent level $\alpha$ test.

\begin{thm}
    We have
    \begin{align*}
        \lim_{n \to \infty} \P{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_{k}}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n} = \begin{cases}
            0,& \text{ if } \norm{\mu}^2 < \Delta,\\
            1,& \text{ if } \norm{\mu}^2 > \Delta \text{ and } \sum_{k=1}^d \innpr{\mu, v_k}^2 > \Delta.
        \end{cases}
    \end{align*}
    and if $\norm{\mu}^2 = \Delta$ and $\sigma^2 > 0$ then
    \begin{align*}
        \lim_{n \to \infty} \P{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_{k}}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n} \leq \alpha.
    \end{align*}
\end{thm}

\begin{proof}
    By the continuous mapping theorem, we can map
    \begin{align*}
        \lambda \longmapsto \sqrt{n} \sum_{k=1}^d \br{\innpr{\overline{X}_{\gbr{n \lambda}}, \hat{v}_{k, \lambda}}^2 - \lambda^2 \innpr{\mu, v_k}^2 }
    \end{align*}
    under the function
    \begin{align*}
        f \longmapsto \frac{f(1)}{\br{\int_0^1 \br{f(\lambda) - \lambda^2 f(1) }^2 \mathrm{d}\nu (\lambda) }^{1/2}}
    \end{align*}
    and obtain
    \begin{align}\label{disp:convergence_for_boundedness}
        \frac{\sqrt{n} \sum_{k=1}^d \br{\innpr{\overline{X}_n , \hat{v}_k}^2 - \innpr{\mu, v_k}^2} }{ \sqrt{n}  \hat{\mathbb{V}}_n} \convd \frac{\mathbb{B}(1)}{\br{\int_0^1 \lambda^2 \br{ \mathbb{B} (\lambda) - \lambda \mathbb{B}(1) }^2 \mathrm{d}\nu (\lambda) }^{1/2}} = \mathbb{W}.
    \end{align}
    Now, first consider the case $\norm{\mu}^2 < \Delta$. We can rewrite the expression as follows
    \begin{align*}
        &\P{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n}\\
        &\pppad\pppad = \P{ \frac{ \sqrt{n} \sum_{k=1}^d \br{\innpr{\overline{X}_n, \hat{v}_k}^2 - \innpr{\mu, v_k}^2}}{\sqrt{n} \hat{\mathbb{V}}_n} > \frac{ \sqrt{n} \br{\Delta - \sum_{k=1}^d \innpr{\mu, v_k}^2}}{\sqrt{n} \hat{\mathbb{V}}_n} + q_{1-\alpha} (\mathbb{W})}.
    \end{align*}
    By Parseval's identity, $\sqrt{n} \br{\Delta - \sum_{k=1}^d \innpr{\mu, v_k}^2} > \sqrt{n} \br{\Delta - \norm{\mu}^2 } \conv \infty$ and since $\sqrt{n} \hat{\mathbb{V}}_n = O_\p (1)$, the right hand side becomes arbitrarily large and therefore in combination with (\ref{disp:convergence_for_boundedness})
    \begin{align*}
        \P{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n} \conv 0.
    \end{align*}
    If $\norm{\mu}^2 = \Delta$, we have by Parseval's identity
    \begin{align*}
        \P{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n} \leq \P{\frac{ \sqrt{n} \sum_{k=1}^d \br{\innpr{\overline{X}_n, \hat{v}_k}^2 - \innpr{\mu, v_k}^2}}{\sqrt{n} \hat{\mathbb{V}}_n} >  q_{1-\alpha} (\mathbb{W})} = \alpha.
    \end{align*}
    Lastly, if $\norm{\mu}^2 > \Delta$ and $\sum_{k=1}^d \innpr{\mu, v_k}^2 > \Delta$, we can use $\sqrt{n} \hat{\mathbb{V}}_n = O_\p (1)$ and $\Delta - \sum_{k=1}^d \innpr{\mu, v_k}^2 < 0$ to obtain
    \begin{align*}
        \P{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n} &= \P{ \frac{\sqrt{n} \sum_{k=1}^d \br{ \innpr{\overline{X}_n, \hat{v}_k}^2 - \innpr{\mu, v_k}^2 }}{\sqrt{n} \hat{\mathbb{V}_n}} > \frac{\sqrt{n} \br{\Delta - \sum_{k=1}^d \innpr{\mu, v_k}^2} }{\sqrt{n} \hat{\mathbb{V}}_n} + q_{1-\alpha} (\mathbb{W}) }\\
        &= \P{O_\p (1) > O_\p (- \sqrt{n}) } \conv 1.
    \end{align*}
\end{proof}

\begin{rem}
    \begin{enumerate}
        \item \blue{ The condition that $\sum_{k=1}^d \innpr{\mu, v_k}^2 > \Delta$ cannot be removed from the last case, as otherwise consistency cannot be achieved. Because if we assume that $\sum_{k=1}^d \innpr{\mu, v_k}^2 \leq \Delta$, then we have
        \begin{align*}
            \P{ \sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}_n} } &= \P{ \frac{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_k}^2 - \sum_{k=1}^d \innpr{\mu, v_k}^2}{\hat{\mathbb{V}}_n} > \frac{\Delta - \sum_{k=1}^d \innpr{\mu, v_k}^2}{\hat{\mathbb{V}}_n} + q_{1-\alpha} (\mathbb{W}) }\\
            &\leq \P{O_\p (1) > q_{1-\alpha} (\mathbb{W}) } = \alpha.
        \end{align*}
        }
        \item Because of 1. it makes sense to test the hypotheses
        \begin{center}
            $H_0: \sum_{k=1}^d \innpr{\mu, v_k}^2 \leq \Delta$ vs. $H_1 : \sum_{k=1}^d \innpr{\mu, v_k}^2 > \Delta$,
        \end{center}
        which yield< the result
        \begin{align*}
            \lim_{n \to \infty} \P{\sum_{k=1}^d \innpr{\overline{X}_n, \hat{v}_k}^2 > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n} = \begin{cases}
                0,& \text{ if } \sum_{k=1}^d \innpr{\mu, v_k}^2 < \Delta,\\
                \alpha,& \text{ if } \sum_{k=1}^d \innpr{\mu, v_k}^2 = \Delta \text{ and } \sigma^2 > 0,\\
                1,& \text{ if } \sum_{k=1}^d \innpr{\mu, v_k}^2 > \Delta
            \end{cases}
        \end{align*}
        for the decision rule proposed in (\ref{decision_rule_proj_onesample}).
    \end{enumerate}
\end{rem}

==> spatiotemporal_cp_mean.tex <==
Consider data following the model
\begin{align*}
    X_i = \begin{cases}
        \mu  + f_1 (\varepsilon_i, \varepsilon_{i-1}, ...), & i \leq n \vartheta_0,\\
        \mu + \delta + f_2 (\varepsilon_i, \varepsilon_{i-1}, ...), & i > n \vartheta_0,
    \end{cases}
\end{align*}
where $\mu, \delta$ denote deterministic, but unknown elements in $L^2 (S \times \sqbr{0,1})$ and $\vartheta_0 \in \br{0,1}$ is the true (unknown) changepoint. Define for $s \in S$ and $t \in \sqbr{0,1}$ $$S_n (s, t, \lambda) := \frac{1}{n} \sum_{i=1}^{\gbr{n \lambda}} \br{X_i (s,t) - \mu (s,t)}$$

To state our next result, we need the following Theorem, which one obtains from generalizing Theorem 1 in \cite{berkes}.

\begin{thm}\label{generalberkes}
    Assumption \ref{ass_2nd} is satisfied. For any $n \in \mathbb{N}$, we can define a family of Gaussian processes $\cbr{\Gamma_n (s, t, \lambda) \mid s \in S, 0 \leq \lambda, t \leq 1}$ such that
    \begin{align*}
        \sup_{0 \leq \lambda \leq 1} \sum_{s \in S} \int \br{ \sqrt{n} S_n (s, t, \lambda) - \Gamma_n (s, t, \lambda)}^2 \mathrm{d}t = \sup_{0 \leq \lambda \leq 1} \norm{\sqrt{n} S_n (\cdot, \cdot, \lambda) - \Gamma_n (\cdot, \cdot, \lambda)}^2 = o_\p (1)
    \end{align*}
    and $\cbr{\Gamma_n (s, t, \lambda) \mid s \in S, 0 \leq \lambda, t \leq 1} \eqo{$\mathpcal{D}$} \cbr{\Gamma (s, t, \lambda) \mid s \in S, 0 \leq \lambda, t \leq 1}$ with $$\Gamma (s, t, \lambda) := \sum_{i=1}^\infty \sqrt{\lambda_i} \phi(s, t) W_i (\lambda).$$ $\lambda_i, \phi_i$ are the eigenvalues and eigenvectors of the covariance operator of $\cbr{X_j}_{j \in \mathbb{Z}}$ and $W_i$ are independent and identically distributed standard Brownian motions.
\end{thm}


%% construction of change point estimator
Next, we need to define an estimator for the unknown change point $\vartheta_0$. For this, we use the following
\begin{align}\label{def_changepoint_estimator}
    \hat{\vartheta} := \frac{1}{n} \argmax_{ \gbr{n \varepsilon} +1 \leq k \leq n - \gbr{n \varepsilon}} f(k),
\end{align}
where $$f(k) := \frac{k(n-k)}{n^2} \norm{\frac{1}{k} \sum_{i=1}^k X_i - \frac{1}{n-k} \sum_{i=k+1}^n X_i }^2.$$ The next result shows that this estimator is consistent for $\vartheta_0$. The proof is omitted, since it goes by the same argumentation as in Proposition 3.1 in \cite{dette}.

\begin{prop}\label{prop:changepoint_conv_rate}
    If $\cbr{X_j}_{j \in \mathbb{Z}}$ satisfies assumption \ref{ass_2nd}, $\norm{\delta}^2 >0$, $\vartheta_0 \in (\varepsilon, 1- \varepsilon)$, then $$\hat{\vartheta} = \vartheta_0 + o_\p (n^{-1/2}).$$
\end{prop}





To state the next result, we need to define the quantities
\begin{align*}
    D_n (s, t, \lambda, \vartheta) := \frac{1}{\gbr{n \vartheta}} \sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta}}} X_j (s, t) - \frac{1}{n - \gbr{n \vartheta}} \sum_{j=\gbr{n \vartheta} + 1}^{\gbr{n \vartheta} + \gbr{\lambda (n - \gbr{n \vartheta})}} X_j (s,t)
\end{align*}
and
\begin{align*}
    \tilde{D}_n (s, t, \lambda, \vartheta) & := \frac{1}{\gbr{n \vartheta}} \sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta}}} \eta^{(1)}_j (s, t) - \frac{1}{n - \gbr{n \vartheta}} \sum_{j=\gbr{n \vartheta} + 1}^{\gbr{n \vartheta} + \gbr{\lambda (n - \gbr{n \vartheta})}} \eta^{(2)}_j (s,t).
\end{align*}
We further denote by $D_n(\lambda, \vartheta)$ and $\tilde{D}_n (\lambda, \vartheta)$ the corresponding element in $L^2 (S \times T)$. Moreover, the equality $D_n (\lambda, \vartheta) + \lambda \delta = \tilde{D}_n (\lambda, \vartheta) + O_\p (n^{-1})$ holds.


\blue{
\begin{lem}\label{lem:approx_for_cp_in_summation}
    If assumption \ref{ass_2nd} is true, then
    \begin{enumerate}
        \item $\displaystyle \sup_{0 \leq \lambda \leq 1} \norm{D_n (\lambda, \vartheta)} = O_\p (1)$ for $\vartheta \in \{ \vartheta_0, \hat{\vartheta} \}$ \red{(eigentlich benötigt man nur $\vartheta_0$; erst in Kap. 3 benötigt)},
        \item $\displaystyle \sup_{0 \leq \lambda \leq 1} \norm{D_n (\lambda, \hat{\vartheta}) - D_n (\lambda, \vartheta_0) } = o_\p (n^{-1/2})$.
    \end{enumerate}
\end{lem}
}

\blue{
\begin{proof}
    We can assume that $\frac{1}{n} \leq \lambda$, because if $0 \leq \lambda < \frac{1}{n}$, by definition $D_n (\lambda, \vartheta) \equiv 0$ for $\vartheta \in \{ \vartheta_0, \hat{\vartheta} \}$ and both assertions are trivially true.
    \begin{enumerate}
        \item In the following, we need a slight variation of Lemma B.1 from the online supplementary material of \cite{aue2}, which states that
        \begin{align}\label{disp:aue_lemma_b1}
            \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\sqrt{\gbr{\lambda n}}} \norm{\sum_{j=1}^{\gbr{\lambda n}} \eta_j} = O_\p (\log^{1/\kappa} (n))
        \end{align}
        for centered $L^2 (S \times \sqbr{0,1})$-valued random variables $\cbr{\eta_j}_{j \in \mathbb{Z}}$. Let $\vartheta \in \{ \vartheta_0, \hat{\vartheta} \}$ and $\lambda \in \sqbr{1/n, 1}$, then $$\norm{D_n (\lambda, \vartheta)} \leq \norm{\tilde{D}_n (\lambda, \vartheta)} + \lambda \norm{\delta} + o_\p (1) = \norm{\tilde{D}_n (\lambda, \vartheta)} + O_\p (1).$$
        Next, we will show that $\norm{\tilde{D}_n (\lambda, \vartheta)} = o_\p (1)$, from which the assertion follows. We have
        \begin{align*}
            \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\tilde{D}_n (\lambda, \vartheta)} \leq \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\gbr{n \vartheta}} \norm{\sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta}}} \eta_j^{(1)} } + \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{n - \gbr{n \vartheta}} \norm{\sum_{j=\gbr{n \vartheta} +1 }^{\gbr{n \vartheta} + \gbr{\lambda (n - \gbr{n \vartheta})}} \eta_j^{(2)} },
        \end{align*}
        where we now only consider the first term, since both calculations are similar. We have
        \begin{align*}
            \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\gbr{n \vartheta}} \norm{\sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta}}} \eta_j^{(1)} } &\leq \frac{1}{\sqrt{\gbr{n \vartheta}}} \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\sqrt{\gbr{\lambda \gbr{n \vartheta}}}} \norm{\sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta}}} \eta_j^{(1)} }\\
            &\leq \frac{1}{\sqrt{\gbr{n \vartheta}}} \sup_{\frac{1}{n} \leq \lambda \leq 1} \frac{1}{\sqrt{\gbr{\lambda n}}} \norm{\sum_{j=1}^{\gbr{\lambda n}} \eta_j^{(1)} } = O_\p \br{\frac{\log^{1/\kappa} (n)}{\sqrt{n}}} = o_\p (1).
        \end{align*}
        In the last inequality, we expanded the set over which we take the supremum and in the last step, we used the convergence rate in (\ref{disp:aue_lemma_b1}).
        %%%%%%%%%%%%%
        \item In this step, we need the following (slightly more general) statement from the beginning of chapter B.1 in \cite{dette}, which states that for the process $\cbr{\Gamma_n (s, t, \lambda) \mid s \in S, 0 \leq t, \lambda \leq 1}$ and a positive sequence $\br{\kappa_n}_{n \in \mathbb{N}}$ with $\kappa_n \to 0$, we have
        \begin{align}\label{disp:sup_gamma_cont}
            \sup_{\substack{\nu, \lambda \in \sqbr{0,1}:\\ |\nu - \lambda| \leq \kappa_n}} \norm{\Gamma_n (\cdot, \cdot, \nu) - \Gamma_n (\cdot, \cdot, \lambda)}^2 = o_\p (1).
        \end{align}
        By adding and subtracting $\lambda \delta$, we have $D_n (\lambda, \hat{\vartheta}) - D_n (\lambda, \vartheta_0) = \tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0) + O_\p (n^{-1})$. Further rewriting yields
        \begin{align*}
            \tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0) &= \frac{1}{\gbr{n \hat{\vartheta}}} \sum_{j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_j^{(1)} - \frac{1}{\gbr{n \vartheta_0}} \sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta_0}}} \eta_j^{(1)}\\
            &\pppad+ \frac{1}{n - \gbr{n \hat{\vartheta}}} \sum_{j=\gbr{n \hat{\vartheta}} + 1}^{\gbr{n \hat{\vartheta}} + \gbr{\lambda (n - \gbr{n \hat{\vartheta}}) }} \eta_j^{(2)} - \frac{1}{n - \gbr{n \vartheta_0}} \sum_{j=\gbr{n \vartheta_0} + 1}^{\gbr{n \vartheta_0} + \gbr{\lambda (n - \gbr{n \vartheta_0}) }} \eta_j^{(2)}
        \end{align*}
        and similarly as above, we only consider the first difference. Expanding the set over which we take the supremum leads to
        \begin{align*}
            &\sup_{\frac{1}{n} \leq \lambda \leq 1} \sqrt{n} \norm{\frac{1}{\gbr{n \hat{\vartheta}}} \sum_{j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_j^{(1)} - \frac{1}{\gbr{n \vartheta_0}} \sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta_0}}} \eta_j^{(1)} }\\
            &\pppad\leq \frac{n}{\gbr{n \hat{\vartheta}}} \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\frac{1}{\sqrt{n}}  \sum_{j=1}^{\gbr{\lambda \gbr{n \hat{\vartheta}}}} \eta_j^{(1)} - \Gamma_n \br{\cdot, \cdot, \lambda \tfrac{\gbr{n \hat{\vartheta}}}{n}}} + \frac{n}{\gbr{n \vartheta_0}} \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\frac{1}{\sqrt{n}}  \sum_{j=1}^{\gbr{\lambda \gbr{n \vartheta_0}}} \eta_j^{(1)} - \Gamma_n \br{\cdot, \cdot, \lambda \tfrac{\gbr{n \vartheta_0}}{n}}} \\
            &\pppad\pppad + \frac{n}{\gbr{n \hat{\vartheta}}} \sup_{\frac{1}{n} \leq \lambda \leq 1}  \norm{\Gamma_n \br{\cdot, \cdot, \lambda \tfrac{\gbr{n \hat{\vartheta}}}{n} } - \Gamma_n (\cdot, \cdot, \lambda \hat{\vartheta})} + \frac{n}{\gbr{n\vartheta_0}} \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{\Gamma_n \br{\cdot, \cdot, \lambda \tfrac{\gbr{n \vartheta_0}}{n}} - \Gamma_n (\cdot, \cdot, \lambda \vartheta_0)}\\
            &\pppad\pppad + \sup_{\frac{1}{n} \leq \lambda \leq 1} \norm{ \frac{n}{\gbr{n \hat{\vartheta}}} \Gamma_n (\cdot, \cdot, \lambda \hat{\vartheta}) - \frac{n}{\gbr{n \vartheta_0}} \Gamma_n (\cdot, \cdot, \lambda \vartheta_0)}\\
            &\pppad\leq \sup_{\substack{\nu, \lambda \in \sqbr{0,1}:\\ |\nu - \lambda| \leq \frac{1}{n}}} \norm{\Gamma_n (\cdot, \cdot, \nu) - \Gamma_n (\cdot, \cdot, \lambda)} + O(1) \negthickspace \negthickspace \sup_{\substack{\nu, \lambda \in \sqbr{0,1}:\\|\nu - \lambda| \leq |\hat{\vartheta} - \vartheta_0|}} \norm{\Gamma_n (\cdot, \cdot, \nu) - \Gamma_n (\cdot, \cdot, \lambda) } + \frac{|\vartheta_0 - \hat{\vartheta}|}{\vartheta_0 \hat{\vartheta}} O_\p (1) +  o_\p (1)\\
            &\pppad= o_\p (1),
        \end{align*}
        where in the last equality we have used (\ref{disp:sup_gamma_cont}). From this the second assertion follows.
    \end{enumerate}
\end{proof}
}


\begin{thm}\label{thm:cp_spatiotemporal_mean}
    Let 
    \begin{align*}
        \tau_{\delta, \vartheta_0}^2 := 4 \sum_{s_1, s_2 \in S} \int \negthickspace \int \delta(s_1, t_1) \delta(s_2, t_2) \br{\tfrac{1}{\vartheta_0} K_1 ((s_1, t_1) , (s_2, t_2))) + \tfrac{1}{1-\vartheta_0} K_2 ((s_1, t_1) , (s_2, t_2))} \mathrm{d}t_1 \mathrm{d}t_2,
    \end{align*}
    where
    \begin{align*}
        K_i ((s_1, t_1), (s_2, t_2)) := \sum_{h \in \mathbb{Z}} \cov (\eta^{(i)}_0 (s_1, t_1), \eta^{(i)}_h (s_2, t_2))
    \end{align*}
    are the long-run covariance kernels of $\{\eta^{(i)}_j\}_{j \in \mathbb{Z}}$ for $i=1,2$. If assumption \ref{ass_2nd} is satisfied, the following statements are true.
    \begin{enumerate}
        \item As $n \to \infty$ $$\sqrt{n} \br{\norm{D_n (\lambda, \vartheta_0)}^2 - \lambda^2 \norm{\delta}^2} \convproc \tau_{\delta, \vartheta_0} \cbr{\lambda \mathbb{B}(\lambda)}_{\lambda \in \sqbr{0,1}}.$$
        
        
        \item Replacing $\vartheta_0$ by $\hat{\vartheta}$ gives the same result, i.e. as $n \to \infty$ $$\sqrt{n} \br{\norm{D_n (\lambda, \hat{\vartheta})}^2 - \lambda^2 \norm{\delta}^2} \convproc \tau_{\delta, \vartheta_0} \cbr{\lambda \mathbb{B}(\lambda)}_{\lambda \in \sqbr{0,1}}.$$
    \end{enumerate}
\end{thm}


% \red{
% \begin{lem}\label{general_lemma_b1}
%     Let $\zeta_1 \in L^2 (S \times \sqbr{0,1})$, $\zeta_2 \in L^2 ((S \times \sqbr{0,1})^2)$ be fixed but arbitrary functions, $\lambda \in \sqbr{0,1}$ and for $\eta_i := X_i - \mu$ define
%     \begin{align*}
%         \tilde{Z}_n^{(1)} (\lambda) := \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{n \lambda}} \innpr{\eta_i, \zeta_1} \pppad \text{ and } \pppad \tilde{Z}_n^{(2)} (\lambda) := \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{n \lambda}} \innpr{\eta_i \otimes \eta_i - c, \zeta_2}_2.
%     \end{align*}
%     Then if assumption \ref{ass_4th} holds, we have the convergence in $\ell^{\infty} (\sqbr{0,1})^2$
%     \begin{align*}
%         \br{\tilde{Z}_n^{(1)}, \tilde{Z}_n^{(2)}} \convproc \Sigma^{\nicefrac{1}{2}} \br{\mathbb{B}_1, \mathbb{B}_2},
%     \end{align*}
%     where $\mathbb{B}_1, \mathbb{B}_2$ are independent Brownian motions and $\Sigma$ is the $2 \times 2$ matrix, defined by the entries
%     \begin{align*}
%         \Sigma_{11} &= \sum_{h \in \mathbb{Z}} \sum_{s_1, s_2 \in S} \int \mathrm{Cov} (\eta_0 (s_1, t_1), \eta_h (s_2, t_2)) \zeta_1 (s_1, t_1) \zeta_1 (s_2, t_2) \mathrm{d} t_1 \mathrm{d} t_2\\
%         \Sigma_{12} &= \sum_{h \in \mathbb{Z}} \sum_{s_1, s_2, s_3 \in S} \int \mathrm{Cov} (\eta_0 (s_1, t_1), \eta_h (s_2, t_2) \eta_h (s_3, t_3)) \zeta_1 (s_1, t_1) \zeta_2 ((s_2, t_2), (s_3, t_3)) \mathrm{d}t_1 \mathrm{d}t_2 \mathrm{d}t_3\\
%         \Sigma_{21} &= \sum_{h \in \mathbb{Z}} \sum_{s_1, s_2, s_3 \in S} \int \mathrm{Cov} (\eta_0 (s_1, t_1) \eta_0 (s_2, t_2), \eta_h (s_3, t_3)) \zeta_2 ((s_1, t_1), (s_2, t_2)) \zeta_1 (s_3, t_3) \mathrm{d}t_1 \mathrm{d}t_2 \mathrm{d}t_3\\
%         \Sigma_{22} &= \sum_{h \in \mathbb{Z}} \sum_{s_1, s_2, s_3, s_4 \in S} \int \mathrm{Cov} (\eta_0 (s_1, t_1) \eta_0 (s_2, t_2), \eta_h (s_3, t_3) \eta_h (s_4, t_4)) \zeta_2 ((s_1, t_1), (s_2, t_2)) \zeta_2 ((s_3, t_3), (s_4, t_4)) \mathrm{d} t_1 \mathrm{d} t_2 \mathrm{d} t_3 \mathrm{d} t_4
%     \end{align*}
%     %\red{possible other notation:
%     %\begin{align*}
%     %    \Sigma_{11} &= \sum_{h \in \mathbb{Z}} \innpr{\xi_{0,h}, \zeta_1 \otimes \zeta_1}_2\\
%     %    \Sigma_{12} &= \sum_{h \in \mathbb{Z}} \innpr{\xi_{0,hh}, \zeta_1 \otimes \zeta_2 }_3\\
%     %    \Sigma_{21} &= \sum_{h \in \mathbb{Z}} \innpr{\xi_{h,00}, \zeta_2 \otimes \zeta_1 }_3\\
%     %    \Sigma_{22} &= \sum_{h \in \mathbb{Z}} \innpr{\xi_{00,hh} \zeta_2 \otimes \zeta_2}_4
%     %\end{align*}
%     %}
% \end{lem}
% }

For the proof of this theorem, we need the following lemma. Its proof is similar to Lemma B.1 in \cite{dette} and is therefore omitted. For the sake of brevity introduce the inner product $\innpr{\cdot, \cdot}_2$ on the space $L^2 (\br{S \times \sqbr{0,1}}^2)$, which is defined as
\begin{align*}
    \innpr{f,g}_2 := \sum_{s_1,s_2 \in S} \int \negthickspace \int f((s_1, t_1), (s_2, t_2)) g((s_1, t_1), (s_2, t_2)) \mathrm{d}t_1 \mathrm{d}t_2
\end{align*}
for $f,g \in L^2 ((S \times \sqbr{0,1})^2)$.

{\color{blue}
\begin{lem}\label{general_lemma_b1}
    Let $\zeta_1, \zeta_2 \in L^2 (S \times \sqbr{0,1})$, $\xi_1, \xi_2 \in L^2 ((S \times \sqbr{0,1})^2)$ be fixed but arbitrary functions, $\lambda \in \sqbr{0,1}$ and for centered processes $\eta^{(1)}, \eta^{(2)}$ {\color{red} with the same $\varepsilon_i, i\in \mathbb{Z}$} that satisfy assumption \ref{ass_4th} define
    \begin{align*}
        \tilde{Z}_n^{(k)} (\lambda) := \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{n \lambda}} \br{\innpr{\eta_i^{(k)} \otimes \eta_i^{(k)}, \xi_k}_2 + \innpr{\eta_i^{(k)}, \zeta_k}}
    \end{align*}
    for $k=1,2$. Then we have the convergence in $\ell^{\infty} (\sqbr{0,1})^2$
    \begin{align*}
        \br{\tilde{Z}_n^{(1)}, \tilde{Z}_n^{(2)}} \convproc \Sigma^{1/2} \br{\mathbb{B}_1, \mathbb{B}_2},
    \end{align*}
    where $\mathbb{B}_1, \mathbb{B}_2$ are independent Brownian motions and $\Sigma$ is the $2 \times 2$ matrix, defined by the entries
    \begin{align*}
        \Sigma_{kl} = \sum_{i\in \mathbb{Z}} &\bigg(\cov (\innpr{\eta_0^{(k)} \otimes \eta_0^{(k)}, \xi_k}_2, \innpr{\eta_i^{(l)} \otimes \eta_i^{(l)}, \xi_l}_2) + \cov (\innpr{\eta_0^{(k)} \otimes \eta_0^{(k)}, \xi_k}_2, \innpr{\eta_i^{(l)}, \zeta_l})\\
        & \pad  +\cov (\innpr{\eta_0^{(k)}, \zeta_k}, \innpr{\eta_i^{(l)} \otimes \eta_i^{(l)}, \xi_l}_2) + \cov (\innpr{\eta_0^{(k)}, \zeta_k}, \innpr{\eta_i^{(l)}, \zeta_l}) \bigg)
    \end{align*}
\end{lem}
}

\begin{proof}[Proof of Theorem \ref{thm:cp_spatiotemporal_mean}]
    \begin{enumerate}
        \item  Using $D_n (\lambda, \vartheta) + \lambda \delta = \tilde{D}_n (\lambda, \vartheta) + O_\p (n^{-1})$, we have by several applications of the Cauchy-Schwarz inequality
            \begin{align*}
                \sqrt{n} \br{\norm{D_n (\lambda, \vartheta_0)}^2 - \lambda^2 \norm{\delta}^2} &= \tfrac{1}{\sqrt{n}} \norm{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0)}^2 + 2\lambda \innpr{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0), \delta} + o_\p (1)\\
                &= 2\lambda \innpr{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0), \delta} + o_\p (1),
            \end{align*}
            since $\norm{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0)}^2 = O_\p (1)$ by Theorem \ref{generalberkes}. Next define for $i=1,2$ and $\lambda \in \sqbr{0,1}$
            \begin{align*}
                \tilde{Z}^{(i)}_n (\lambda) := \frac{1}{\sqrt{n}} \sum_{j=1}^{\gbr{\lambda n}} \innpr{\eta_j^{(i)}, \delta},
            \end{align*}
            in order to rewrite
            \begin{align*}
                \innpr{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0), \delta} &= \frac{n}{\gbr{n \vartheta_0}} \frac{1}{\sqrt{n}} \sum_{i=1}^{\gbr{\lambda \gbr{n \vartheta_0}}} \innpr{ \eta_i^{(1)} , \delta} - \frac{n}{n - \gbr{n \vartheta_0}} \frac{1}{\sqrt{n}} \sum_{i=\gbr{n \vartheta_0} + 1}^{\gbr{n \vartheta_0} + \lambda (n - \gbr{n \vartheta_0})} \innpr{ \eta_i^{(2)} , \delta}\\
                &= \frac{n}{\gbr{n \vartheta_0}} \tilde{Z}^{(1)}_n \br{\lambda \tfrac{\gbr{n \vartheta_0}}{n}} - \frac{n}{n - \gbr{n \vartheta_0}} \br{\tilde{Z}^{(2)}_n \br{\tfrac{\gbr{n \vartheta_0} + \gbr{\lambda (n - \gbr{n \vartheta_0})}}{n}} - \tilde{Z}^{(2)}_n \br{\vartheta_0}}.
            \end{align*}
            Hence,
            \begin{align*}
                \sqrt{n} \br{\norm{D_n (\lambda, \vartheta_0)}^2 - \lambda^2 \norm{\delta}^2} = \frac{2 \lambda}{\vartheta_0} \tilde{Z}^{(1)}_n \br{\lambda \tfrac{\gbr{n \vartheta_0}}{n}} - \frac{2 \lambda}{1-\vartheta_0} \br{\tilde{Z}^{(2)}_n \br{\tfrac{\gbr{n \vartheta_0} + \gbr{\lambda (n - \gbr{n \vartheta_0})}}{n}} - \tilde{Z}^{(2)}_n \br{\vartheta_0}} + o_\p (1)
            \end{align*}
            and by an application of Lemma \ref{general_lemma_b1} with $\zeta_1 = \zeta_2 = \delta$ and $\xi_1 = \xi_2 \equiv 0$, we obtain
            \begin{align*}
                \cbr{\sqrt{n} \br{\norm{D_n (\lambda, \vartheta_0)}^2 - \lambda^2 \norm{\delta}^2}}_{\lambda \in \sqbr{0,1}} \convproc \cbr{\frac{2 \lambda}{\vartheta_0} \tilde{\mathbb{Z}}^{(1)} (\lambda \vartheta_0) - \frac{2\lambda}{1-\vartheta_0} \br{\tilde{\mathbb{Z}}^{(2)} (\vartheta_0 + \lambda (1- \vartheta_0)) - \tilde{\mathbb{Z}}^{(2)} (\vartheta_0)}}_{\lambda \in \sqbr{0,1}},
            \end{align*}
            with
            \begin{align*}
                \tilde{\mathbb{Z}}^{(1)} = \tilde{\Sigma}_{11} \mathbb{B}_1 + \tilde{{\Sigma}}_{12} \mathbb{B}_2 \pad \pad \pad \tilde{\mathbb{Z}}^{(2)} = \tilde{\Sigma}_{21} \mathbb{B}_1 + \tilde{\Sigma}_{22} \mathbb{B}_2,
            \end{align*}
            where $\mathbb{B}_i$ are Brownian motions, $\tilde{\Sigma}_{ij}$ denotes the $ij$-th entry of $\Sigma^{1/2}$ for $i,j=1,2$ and
            \begin{align*}
                \Sigma = \br{\Sigma_{ij}}_{i,j =1,2} = \br{\sum_{h \in \mathbb{Z}} \sum_{s \in S} \int \negthickspace \int \cov (\eta_0^{(i)} (s_1, t_1), \eta_h^{(j)} (s_2, t_2) ) \delta(s_1, t_1) \delta (s_2, t_2) \mathrm{d}t_1 \mathrm{d}t_2 }_{i,j=1,2}.
            \end{align*}
            Inspecting the covariance structure of the limit above, we see that because of
            \begin{align*}
                \cov (\tilde{\mathbb{Z}}^{(1)} (\lambda_1 \vartheta_0), \tilde{\mathbb{Z}}^{(1)} (\lambda_2 \vartheta_0)) &= (\lambda_1 \wedge \lambda_2) \vartheta_0 \Sigma_{11},\\
                \cov (\tilde{\mathbb{Z}}^{(2)} (\vartheta_0 + \lambda_1 (1 - \vartheta_0)) - \tilde{\mathbb{Z}}^{(2)} ( \vartheta_0), \tilde{\mathbb{Z}}^{(2)} (\vartheta_0 + \lambda_2 (1 - \vartheta_0)) - \tilde{\mathbb{Z}}^{(2)} (\vartheta_0)) &= (\lambda_1 \wedge \lambda_2) (1-\vartheta_0) \Sigma_{22},\\
                \cov (\tilde{\mathbb{Z}}^{(1)} (\lambda_1 \vartheta_0), \tilde{\mathbb{Z}}^{(2)} (\vartheta_0 + \lambda_2 (1 - \vartheta_0)) - \tilde{\mathbb{Z}}^{(2)} ( \vartheta_0)) &= 0,
            \end{align*}
            the limit has the same distribution as $\cbr{\lambda \tau_{\delta, \vartheta_0} \mathbb{B} (\lambda)}_{\lambda \in \sqbr{0,1}}$ from which the assertion follows.
            %%%%%%%%
            \item \blue{By the same calculation as above, we rewrite as follows
                \begin{align*}
                    \sqrt{n} \br{\norm{D_n (\lambda, \hat{\vartheta})}^2 - \lambda^2 \norm{\delta}^2} = \sqrt{n} \norm{\tilde{D}_n (\lambda, \hat{\vartheta})}^2 + 2 \lambda \sqrt{n} \innpr{\tilde{D}_n (\lambda, \hat{\vartheta}), \delta} + o_\p (1).
                \end{align*}
                By the second assertion of Lemma \ref{lem:approx_for_cp_in_summation} and Theorem \ref{generalberkes}, we have that
                \begin{align*}
                    \norm{\tilde{D}_n (\lambda, \hat{\vartheta})}^2 \leq 2 \sqrt{n} \norm{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0)}^2 + 2 \frac{1}{\sqrt{n}} \norm{ \sqrt{n} \tilde{D}_n (\lambda, \vartheta_0)}^2 = o_\p (1)
                \end{align*}
                and again by Lemma \ref{lem:approx_for_cp_in_summation}
                \begin{align*}
                    2 \lambda \sqrt{n} \innpr{\tilde{D}_n (\lambda, \hat{\vartheta}), \delta} = 2 \lambda \innpr{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0)} + \sqrt{n} 2 \lambda \innpr{\tilde{D}_n (\lambda, \hat{\vartheta}) - \tilde{D}_n (\lambda, \vartheta_0), \delta } = 2 \lambda \innpr{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0)} + o_\p (1)
                \end{align*}
                using the Cauchy-Schwarz inequality. It follows that
                \begin{align*}
                    \sqrt{n} \br{\norm{D_n (\lambda, \hat{\vartheta})}^2 - \lambda^2 \norm{\delta}^2} = 2 \lambda \innpr{\sqrt{n} \tilde{D}_n (\lambda, \vartheta_0), \delta} + o_\p (1)
                \end{align*}
                and we have the same expression as in the first part of the proof, leading to the fact that it weakly converges to the same limiting distribution.}
    \end{enumerate}
\end{proof}

\noindent To test the hypotheses
\begin{center}
    $H_0$: $\norm{\delta}^2 \leq \Delta$ vs. $H_1$: $\norm{\delta}^2 > \Delta$
\end{center}
for $\Delta > 0$ we define
\begin{align*}
    \hat{\mathbb{D}}_n &:= \norm{D_n (1, \hat{\vartheta})}^2\\
    \hat{\mathbb{V}}_n &:= \br{\int \br{\norm{D_n (\lambda, \hat{\vartheta})}^2 - \lambda^2 \norm{D_n (1, \hat{\vartheta})}^2}^2 \mathrm{d} \nu (\lambda) }^{1/2},
\end{align*}
where $\hat{\vartheta}$ is defined as in (\ref{def_changepoint_estimator}) and $\nu$ a probability measure on $(0,1)$. Then, the test takes the following form: Reject $H_0$, if
\begin{align*}
    \hat{\mathbb{D}}_n > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n,
\end{align*}
where $q_{1-\alpha} (\mathbb{W})$ is the $(1-\alpha)$-quantile of the random variable
\begin{align}\label{disp:random_variable_w}
    \mathbb{W} := \frac{\mathbb{B} (1)}{\br{\int \lambda^2 (\mathbb{B}(\lambda) - \lambda \mathbb{B} (1) )^2 \mathrm{d}\nu (\lambda) }^{1/2}}.
\end{align}

\begin{thm}
    Under assumption \ref{ass_2nd}, $\Delta > 0$ \red{and $\vartheta_0 \in \br{\varepsilon, 1- \varepsilon}$}, the decision rule above defines an asymptotic level $\alpha$ test and is consistent. More concretely, this means
    \begin{align*}
        \lim_{n \to \infty} \P{\hat{\mathbb{D}}_n > \Delta + q_{1-\alpha} (\mathbb{W}) \hat{\mathbb{V}}_n} = \begin{cases}
            0,& \text{if } \norm{\delta}^2 < \Delta,\\
            \alpha,& \text{if } \norm{\delta}^2 = \Delta,\\
            1,& \text{if } \norm{\delta}^2 > \Delta.
        \end{cases}
    \end{align*}
\end{thm}

\begin{proof}
    \red{see further down}
\end{proof}
